Multi-Objective-Guided Discrete Flow Matching for Controllable Biological Sequence Design

Designing biological sequences that satisfy multiple, often conflicting, functional and biophysical criteria remains a central challenge in biomolecule engineering. While discrete flow matching models have recently shown promise for efficient sampling in high-dimensional sequence spaces, existing approaches address only single objectives or require continuous embeddings that can distort discrete distributions. We present Multi-Objective-Guided Discrete Flow Matching (MOG-DFM), a general framework to steer any pretrained discrete flow matching generator toward Pareto-efficient trade-offs across multiple scalar objectives. At each sampling step, MOG-DFM computes a hybrid rank-directional score for candidate transitions and applies an adaptive hypercone filter to enforce consistent multi-objective progression. We also trained two unconditional discrete flow matching models, PepDFM for diverse peptide generation and EnhancerDFM for functional enhancer DNA generation, as base generation models for MOG-DFM. We demonstrate MOG-DFM's effectiveness in generating peptide binders optimized across five properties (hemolysis, non-fouling, solubility, half-life, and binding affinity), and in designing DNA sequences with specific enhancer classes and DNA shapes. In total, MOG-DFM proves to be a powerful tool for multi-property-guided biomolecule sequence design.

==> Tables/5_classifiers_examples.tex <==
\begin{table}[ht]
\centering
\caption{Representative MOG-DFM-designed binders selected for each target. The affinity scores are predicted by the score model, while the ipTM and VINA scores are predicted by AlphaFold3 and AutoDock VINA.}
\vspace{0.5em}
% \small
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Target} & \textbf{Example} & \textbf{Affinity} & \textbf{ipTM} & \textbf{VINA} \\
\hline
AMHR2       & DAEAWVEV         & 8.74  & 0.87 & -6.0  \\
AMHR2       & DYAMRTRRRRWG     & 8.64  & 0.90 & -6.3  \\
AMHR2       & PFRAEEDLGEEVEVHC& 8.69& 0.77& -6\\
EWS:FLI1    & EVIVWWVIC        & 8.18  & 0.72 & -6.0  \\
EWS:FLI1    & WKKFMAWIVRDG     & 8.36  & 0.70 & -6.7  \\
EWS:FLI1    & EVTYTSVFAQAVAIVC& 8.03& 0.67& -5.5 \\
MYC         & VAKWVRVRP        & 7.93  & 0.55 & -6.6  \\
OX1R        & EWDEKEEAEV       & 10.17 & 0.52 & -8.2  \\
DUSP12      & ESTRWPRVC        & 7.86  & 0.42 & -7.3  \\
 1B8Q& TVVCAAAE& 6.32& 0.6&-5.2\\
 1E6I        & FFWAGV           & 6.31  & 0.73 &-7.2  \\
3IDJ& DFVAAGV& 8.04& 0.75& -7.2\\
5AZ8        & AVWWKFIVYAA & 7.32& 0.74& -9.3\\
7JVS        & WMLWCITWGTC      & 7.94  & 0.56 & -7.3  \\
\hline
\end{tabular}

\label{tab:examples}
\end{table}


==> Tables/existing_binders.tex <==
\begin{table}[ht]
\centering
\midfootnotesize
\caption{MOG-DFM designs peptide binders with significantly improved properties compared to pre-existing binders for each target. Each target is represented by two rows: the upper row shows the amino acid sequence and property scores for the MOG-DFM-designed binders, while the lower row corresponds to the pre-existing binders. AutoDock VINA docking scores are also included to confirm binding affinity.}
\vspace{0.5em}
\begin{tabular}{c|c|cccccl}
\hline
\textbf{PDB ID} & \textbf{Binder} & \textbf{Hemolysis ($\downarrow$)} & \textbf{Non-Fouling} & \textbf{Solubility} & \textbf{Half-Life} & \textbf{Affinity}  &\textbf{VINA}\\ \hline
 \multirow{2}{*}{1B8Q} & TVVCAAAE & 0.0600& 0.9345 & 0.9206 & 80.386&6.0977  &-5.2
\\
 & VVKVDSV& 0.1702 & 0.5678 & 0.3501 & 0.608&4.9273  &-5.1
\\
\hline
\multirow{2}{*}{1E6I} & FFWAGV & 0.1369 & 0.7574 & 0.4547 & 57.667& 6.1304  &-7.2
\\
& AKRHR& 0.0903 & 0.2685 & 0.4333 & 1.866& 4.1409  &-7.4
\\ \hline
\multirow{2}{*}{3IDJ} & DFVAAGV & 0.1267 & 0.7784 & 0.7701 & 92.644 & 8.0048  &-7.2
\\
& ELDAWAS& 0.2100& 0.2094 & 0.2283 & 41.956& 7.0982  &-6.3
\\ \hline
\multirow{2}{*}{5AZ8} & AVWWKFIVYAA & 0.1332 & 0.7551 & 0.5938 & 90.776& 7.3299  &-9.3
\\
& PRLSRLLSYAG& 0.1289 & 0.0945 & 0.1308 & 0.607& 6.1569  &-7.2
\\ \hline
\multirow{2}{*}{7JVS}& WMLWCITWGTC & 0.1253 & 0.5942 & 0.6761& 39.705& 7.9403  &-7.3
\\
& KLNLQFFASKK& 0.2398 & 0.3184 & 0.2010& 0.841& 6.1645  &-5.5\\ \hline
\end{tabular}
\label{tab:existing}
\end{table}
